MANER: Mask Augmented Named Entity Recognition for Extreme Low-Resource Languages

This paper investigates the problem of Named Entity Recognition (NER) for extreme low-resource languages with only a few hundred tagged data samples. NER is a fundamental task in Natural Language Processing (NLP). A critical driver accelerating NER systems' progress is the existence of large-scale language corpora that enable NER systems to achieve outstanding performance in languages such as English and French with abundant training data. However, NER for low-resource languages remains relatively unexplored. In this paper, we introduce Mask Augmented Named Entity Recognition (MANER), a new methodology that leverages the distributional hypothesis of pre-trained masked language models (MLMs) for NER. The <mask> token in pre-trained MLMs encodes valuable semantic contextual information. MANER re-purposes the <mask> token for NER prediction. Specifically, we prepend the <mask> token to every word in a sentence for which we would like to predict the named entity tag. During training, we jointly fine-tune the MLM and a new NER prediction head attached to each <mask> token. We demonstrate that MANER is well-suited for NER in low-resource languages; our experiments show that for 100 languages with as few as 100 training examples, it improves on state-of-the-art methods by up to 48% and by 12% on average on F1 score. We also perform detailed analyses and ablation studies to understand the scenarios that are best-suited to MANER.

==> sections/methodology_old.tex <==
Todos:
\begin{enumerate}
    \item Strategy 2 should have training and inference step information for remark comment in next item; training should be mention word level prepend technique
    \item Remove strategy 2 - parts of it get moved to i) intuition for strategy ii) why it does not work as a remark after strategy 2 iii) to experiments as a baseline
    \item remark: practical constraints
    \item Intuition needs to include some data to convince people \mask does encode token - replace loc in S with loc from mask, predict those mask from an ner, plot the distribution for many such S
\end{enumerate}

In this section, we detail how to repurpose the \mask token for NER training. Two strategies as outlined in figure \ref{fig:method} are used, which are later compared in the experiment section \ref{sec:exp}.

Set of NER labels is given by $\mc{N} = \{0, 1, 2, 3\}$, where $0=N/A$, $1=PER$, $2=LOC$, and $3=ORG$. 
Let a sentence $S$ consisting of $n$ words be $\{w_{0}, w_{1},.., w_{n-1}\}$ with NER labels $L$ as $\{c_{0}, c_{1},.., c_{n-1}\}$ where $c_i \in \mc{N} \,, \ 0 \leq i<n$. 
Let the transformer model be given by $T$ which takes in input a sentence and outputs an embedding for each word in the sentence, $T(\{w_{0}, w_{1},.., w_{n-1}\}) = \{\v{e}_{0}, \v{e}_{1},.., \v{e}_{n-1}\}$, where $\v{e}_i \in \mb{R}^D \,, \ 0 \leq i<n$, and $D$ is embedding dimension.

\textbf{Baseline}: Current NER systems built upon transformer models add a token classification head to top of a transformer model.
The token classification head predicts the NER class of each token in a sentence and its weights are learned during NER fine-tuning.
Though specialized models have been built for popular languages like english, this baseline method remains the de-facto method to train NER models for most languages (especially low-resource languages) to the best of our knowledge \zw{i would put though... at the end}.

The token classification head is a classifier weight matrix $\v{M} \in \mb{R}^{D \times |\mc{N}|}$, where $|\mc{N}|$ is the cardinality of set of NER labels. The matrix takes token embedding as input and output scores for each NER label.
Passing these scores through a softmax provides probabilities, $\v{p}_i \in \mb{R}^{|\mc{N}|}$, for each NER class for token $i$ given by equation:

\begin{equation}
    \v{p}_i = \rm{softmax}\Bigl(\v{M}\bigl(\v{e}_i\bigl)\Bigl).
\end{equation}
% \zw{the above equation: i think the $p$ is for all NER labels? if you want to do $p_i$ i think the r.h.s should be ${\rm softmax}(\cdot)_i$ with an $i$ subscript}
Then, the weights of $\v{M}$ can be learned by minimizing cross-entropy loss.


Now, we will dive into two strategies to repurpose the \mask token for NER fine-tuning. In both the strategies, we change the sentence representation $S$ and corresponding labels $L$, but the base mechanism to use a token classification head remains the same.

\textbf{First Strategy:} Our first strategy to repurpose the \mask token for NER is inspired by masked language modeling (MLM) framework that is used for pre-training of transformer models. 
In MLM, words are predicted using the words surrounding it in the sentence.
Since NER category of a word is also a semantic property of the word, we use the philosophy of MLM for NER fine-tuning.

In MLM pre-training, dataset is preparing by replacing \zw{maybe put italic on replacing to emphasize it?} random words in a sentence with a \mask token with probability given by $p_{mlm}$.
Then, these masked words are predicted using the context information.

Analogous to MLM pre-training, for NER fine-tuning, we randomly replace words in sentence $S$ with \mask token with  probability given by $p_{ner}$.
However, instead of predicting the missing words as is the case with MLM, we predict the NER labels $L$ for each word $w$ in $S$ irrespective of whether the word was replaced by a \mask token or not.
In the case the word was replaced with the \mask token, transformer outputs the \mask token embedding for that word.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{images/strategy2_results.png}
    \caption{F1 scores comparing baseline NER methods against our strategy 2 for 100 low-resource languages in WikiANN dataset that only have 100 training samples each. On average, our strategy 2 gives a significant improvement of \textbf{12\%} compared to baseline as shown in table \ref{tab:ner_main}. \zw{i think the plot you shared in slack might make a more appealing visual. i can help plot that}}
    \label{fig:100_strategy}
\end{figure*}

Thus the modified input to the transformer is $S' = \rm{mask}(S)$, where 
\begin{equation}
    \rm{mask}(w_i) = 
    \begin{cases}

        \text{\mask},& \text{if } p_i \leq p_{ner},\\
        w_i,              & \text{otherwise}
    \end{cases}
\end{equation}
\zw{how do you get $p_i$ and $p_{\rm ner}$ before training?}
where $p_i$ is a random number between $0$ and $1$ generated for $w_i$.
The labels $L$, however, remain the same.
Then, we use the baseline method to use a token classification head given by matrix $\v{M}$ which is fine-tuned on $S'$ and $L$.

\textbf{Second Strategy:} Unlike our first strategy, here we use the \mask token to have access to the word being labelled as well.
To implement this strategy, a \mask token is appended \zw{maybe italic append to emphasize} to beginning of each word in the sentence.
Thus, during fine-tuning, the NER model can learn to fall back on word if context information is not sufficient, or vice versa.

The modified input for this strategy is $S' = \{m, w_{0}, m, w_{1},.., m, w_{n-1}\}$ where $m$ is the \mask token. 
However, in this strategy only the mask tokens adjacent to each word are classified by the token classification head.
The modified labels $L'$ is $\{c_{0}, -1, c_{1}, -1, .., c_{n-1}, -1\}$ where $-1$ indicates that loss is not calculated for those indices.


==> sections/related_work.tex <==
NER for low-resource languages

